Eliciting ambiguity with mixing bets

Preferences for mixing can reveal ambiguity perception and attitude on a single event. The validity of the approach is discussed for multiple preference classes including maxmin, maxmax, variational, and smooth second-order preferences. An experimental implementation suggests that participants perceive almost as much ambiguity for the stock index and actions of other participants as for the Ellsberg urn, indicating the importance of ambiguity in real-world decision-making.

==> cooperation.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 

 & cooperation \\ 
\hline \\[-1.8ex] 
 mixing intensity $(s)$ & $-$0.04 \\ 
  & (0.05) \\ 
  & \\ 
 risk aversion $(s)$ & 0.01 \\ 
  & (0.05) \\ 
  & \\ 
 multiple mixing $(s)$ & 0.02 \\ 
  & (0.05) \\ 
  & \\ 
 probability of cooperation $(s)$ & 0.24$^{***}$ \\ 
  & (0.05) \\ 
  & \\ 
 Constant & 0.54$^{***}$ \\ 
  & (0.05) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 76 \\ 
R$^{2}$ & 0.22 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> order.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\cline{2-8} 
\\[-1.8ex] & \multicolumn{4}{c}{mixing} & \multicolumn{3}{c}{intensity} \\ 
 & risk & ambiguous & stock & social & ambiguous & stock & social \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 typeslider & 0.314$^{***}$ & 0.214$^{***}$ & 0.193$^{***}$ & 0.271$^{***}$ &  &  &  \\ 
  & (0.035) & (0.032) & (0.039) & (0.042) &  &  &  \\ 
  & & & & & & & \\ 
 female & 0.055 & 0.070$^{*}$ & 0.135$^{***}$ & $-$0.020 & 0.063 & 0.103 & 0.048 \\ 
  & (0.035) & (0.036) & (0.040) & (0.043) & (0.050) & (0.084) & (0.085) \\ 
  & & & & & & & \\ 
 risk aversion $(s)$ & 0.001 & $-$0.015 & $-$0.036$^{*}$ & $-$0.025 & $-$0.007 & $-$0.009 & 0.035 \\ 
  & (0.018) & (0.018) & (0.020) & (0.021) & (0.025) & (0.038) & (0.038) \\ 
  & & & & & & & \\ 
 age $(s)$ & $-$0.016 & $-$0.016 & 0.027 & $-$0.016 & 0.020 & 0.0003 & $-$0.020 \\ 
  & (0.017) & (0.017) & (0.018) & (0.020) & (0.023) & (0.038) & (0.037) \\ 
  & & & & & & & \\ 
 topic number & 0.035$^{**}$ & $-$0.064$^{***}$ & $-$0.0004 & $-$0.027 & 0.002 & $-$0.065$^{*}$ & $-$0.023 \\ 
  & (0.015) & (0.016) & (0.016) & (0.017) & (0.023) & (0.037) & (0.030) \\ 
  & & & & & & & \\ 
 quota number within topic & 0.002 & $-$0.010 & $-$0.003 & 0.001 & 0.004 & $-$0.009 & $-$0.002 \\ 
  & (0.011) & (0.011) & (0.013) & (0.013) & (0.016) & (0.026) & (0.025) \\ 
  & & & & & & & \\ 
 Constant & 0.019 & 0.415$^{***}$ & 0.167$^{**}$ & 0.295$^{***}$ & 0.579$^{***}$ & 0.734$^{***}$ & 0.700$^{***}$ \\ 
  & (0.055) & (0.059) & (0.065) & (0.064) & (0.078) & (0.136) & (0.109) \\ 
  & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 623 & 853 & 618 & 539 & 204 & 78 & 76 \\ 
R$^{2}$ & 0.126 & 0.075 & 0.057 & 0.083 & 0.012 & 0.111 & 0.041 \\ 
Adjusted R$^{2}$ & 0.118 & 0.069 & 0.047 & 0.072 & $-$0.013 & 0.050 & $-$0.027 \\ 
Residual Std. Error & 0.397 (df = 616) & 0.467 (df = 846) & 0.440 (df = 611) & 0.441 (df = 532) & 0.314 (df = 198) & 0.312 (df = 72) & 0.300 (df = 70) \\ 
F Statistic & 14.843$^{***}$ (df = 6; 616) & 11.506$^{***}$ (df = 6; 846) & 6.101$^{***}$ (df = 6; 611) & 7.985$^{***}$ (df = 6; 532) & 0.467 (df = 5; 198) & 1.803 (df = 5; 72) & 0.600 (df = 5; 70) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> participant_domain_reg.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{2}{c}{mixing intensity} & \multicolumn{2}{c}{multiple mixing} & \multicolumn{2}{c}{probability} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 ambiguous &  & 0.03 &  & 0.28$^{**}$ &  & 0.03 \\ 
  &  & (0.05) &  & (0.11) &  & (0.03) \\ 
  & & & & & & \\ 
 stock &  & 0.05 &  & 0.24$^{*}$ &  & 0.13$^{***}$ \\ 
  &  & (0.06) &  & (0.13) &  & (0.04) \\ 
  & & & & & & \\ 
 social &  & 0.04 &  & 0.20 &  & 0.08$^{**}$ \\ 
  &  & (0.07) &  & (0.13) &  & (0.04) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Fixed effects & participant & domain & participant & domain & participant & domain \\ 
Observations & 146 & 146 & 146 & 146 & 146 & 146 \\ 
Adjusted R$^{2}$ & 0.46 & $-$0.02 & 0.09 & 0.03 & $-$0.32 & 0.08 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 


==> results_ind.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{7}{c}{\textit{Dependent variable:}} \\ 
\cline{2-8} 
\\[-1.8ex] & ambiguity  & measurement & \multicolumn{5}{c}{ambiguity perception  $l_{j,d}$} \\
 & aversion $\alpha_j$ & error $\sigma_j$ & risk & ambiguous & updated & stock & social \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 risk aversion $(s)$ & 0.28 & $-$0.01$$ & 0.02 & $-$0.005 & $-$0.02 & $-$0.004 & $-$0.03 \\ 
  & (0.18) & (0.01) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) \\ 
  & & & & & & & \\ 
 female & 0.12 & 0.04$$ & 0.02 & 0.10$$ & 0.10$$ & 0.13$$ & 0.06 \\ 
  & (0.36) & (0.01) & (0.04) & (0.04) & (0.03) & (0.04) & (0.04) \\ 
  & & & & & & & \\ 
 age $(s)$ & 0.05 & $-$0.003 & $-$0.02 & $-$0.02 & 0.005 & $-$0.02 & 0.01 \\ 
  & (0.17) & (0.01) & (0.02) & (0.02) & (0.02) & (0.02) & (0.02) \\ 
  & & & & & & & \\ 
 Constant & 1.40$$ & 0.11$$ & 0.16$$ & 0.24$$ & 0.19$$ & 0.19$$ & 0.22$$ \\ 
  & (0.24) & (0.01) & (0.02) & (0.03) & (0.02) & (0.03) & (0.03) \\ 
  & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 88 & 88 & 88 & 88 & 88 & 88 & 88 \\ 
R$^{2}$ & 0.04 & 0.12 & 0.05 & 0.09 & 0.09 & 0.13 & 0.04 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular} 


==> rum_ind_all.tex <==
\begin{tabular}{lrrrrr}
  \hline
variable & zero & positive & mode = zero & mean & reject zero \\ 
  \hline
compound &  & 0.17 &  & -0.05 & 0.27 \\ 
  hedging &  & 0.97 &  & 0.11 & 0.00 \\ 
  insensivity &  & 1.00 &  & 0.85 & 1.00 \\ 
  length ambiguity & 0.41 &  & 0.56 & 0.40 & 0.17 \\ 
  length risk & 0.91 &  & 0.98 & 0.06 & 0.01 \\ 
  length social & 0.26 &  & 0.57 & 0.36 & 0.10 \\ 
  length stock & 0.46 &  & 0.81 & 0.37 & 0.09 \\ 
  sigma &  & 1.00 &  & 16.30 & 1.00 \\ 
  theta & 0.51 & 1.00 & 0.68 & 0.81 & 0.00 \\ 
   \hline
\end{tabular}


==> rum_ind_l.tex <==
\begin{tabular}{rlrrrrr}
  \hline
 & topic & mean & median & quartile.range & reject.zero & prior.update \\ 
  \hline
1 & ambiguity & 0.40 & 0.41 & 0.46 & 0.23 & 0.64 \\ 
  2 & risk & 0.06 & 0.02 & 0.05 & 0.01 & 0.05 \\ 
  3 & social & 0.36 & 0.37 & 0.11 & 0.10 & 0.84 \\ 
  4 & stock & 0.37 & 0.35 & 0.30 & 0.14 & 0.66 \\ 
   \hline
\end{tabular}


==> rum_rep.tex <==
\begin{tabular}{rlrrr}
  \hline
 & parameter & mean & 0.1-quantile & 0.9-quantile \\ 
  \hline
1 & ambiguity & 0.37 & 0.25 & 0.57 \\ 
  2 & social & 0.42 & 0.24 & 0.55 \\ 
  3 & stock & 0.43 & 0.22 & 0.58 \\ 
  4 & theta & 0.85 & 0.22 & 1.60 \\ 
  5 & beta & 0.75 & 0.75 & 0.75 \\ 
  6 & compound & -0.05 & -0.08 & -0.01 \\ 
  7 & hedging & 0.11 & -0.08 & 0.30 \\ 
  8 & risk & 0.21 & 0.01 & 0.37 \\ 
   \hline
\end{tabular}

